Subquadratic Submodular Maximization with a General Matroid Constraint

We consider fast algorithms for monotone submodular maximization with a general matroid constraint. We present a randomized $(1 - 1/e - \epsilon)$-approximation algorithm that requires $\tilde{O}_{\epsilon}(\sqrt{r} n)$ independence oracle and value oracle queries, where $n$ is the number of elements in the matroid and $r \leq n$ is the rank of the matroid. This improves upon the previously best algorithm by Buchbinder-Feldman-Schwartz [Mathematics of Operations Research 2017] that requires $\tilde{O}_{\epsilon}(r^2 + \sqrt{r}n)$ queries. Our algorithm is based on continuous relaxation, as with other submodular maximization algorithms in the literature. To achieve subquadratic query complexity, we develop a new rounding algorithm, which is our main technical contribution. The rounding algorithm takes as input a point represented as a convex combination of $t$ bases of a matroid and rounds it to an integral solution. Our rounding algorithm requires $\tilde{O}(r^{3/2} t)$ independence oracle queries, while the previously best rounding algorithm by Chekuri-Vondr\'{a}k-Zenklusen [FOCS 2010] requires $O(r^2 t)$ independence oracle queries. A key idea in our rounding algorithm is to use a directed cycle of arbitrary length in an auxiliary graph, while the algorithm of Chekuri-Vondr\'{a}k-Zenklusen focused on directed cycles of length two.

==> swap_rounding_in_previous_work.tex <==
\section{Swap Rounding Algorithm in Previous Work}
\label{sec:preimplement}

In this section, we describe the swap rounding algorithm of Chekuri-Vondr\'{a}k-Zenklusen~\cite{chekuri2010dependent} for a matroid base polytope, which we denote \texttt{SwapRound}. 
%%In the swap rounding algorithm of Chekuri-Vondr\'{a}k-Zenklusen~\cite{chekuri2010dependent}, which we denote \texttt{SwapRound},  
In \texttt{SwapRound},  
we are given a vector $x \in B(\M)$ that is represented as a convex combination of 
the characteristic vectors of $t$ bases of $\M$. 
The output is a single basis $S$ of $\M$ such that
$\E[f(S)] \geq F(x)$ for any submodular function $f\colon 2^V \to \mathbb{R}$ and its multilinear extension $F$. 
In each phase of \texttt{SwapRound}, 
we pick up two bases in the representation of $x$ and merge them into a basis. 
By applying this procedure $t-1$ times, \texttt{SwapRound} finally returns a single basis of $\M$; see Algorithm~\ref{alg:swapround}.  


The procedure for merging two bases is denoted by \texttt{MergeBases} (Algorithm \ref{alg:mergebases}). 
The input of \texttt{MergeBases} consists of two bases $B_1$ and $B_2$ together with 
their coefficients $\beta_1$ and $\beta_2$. 
%%In each step of \texttt{MergeBases}, 
In the procedure, until $B_1$ and $B_2$ coincide, 
we repeatedly update $B_1$ and $B_2$ so that $|B_1 \setminus B_2|$ decreases monotonically. 
In each update of $B_1$ and $B_2$, we need a pair of elements $u \in B_1 \setminus B_2$
and $v \in B_2 \setminus B_1$ such that $B_1 + v - u \in \I$ and $B_2 + u - v \in \I$. 
As described in \texttt{UpdateViaStrongBasisExchange} (Algorithm~\ref{alg:update_via_strong_basis_exchange}), 
for such a pair of elements $u$ and $v$, 
we apply $B_1 \gets B_1 + v - u$ with probability $\frac{\beta_2}{\beta_1+\beta_2}$
and apply $B_2 \gets B_2 + u - v$ with the remaining probability. 
Note that, in \texttt{UpdateViaStrongBasisExchange}, 
$B_1$ and $B_2$ are updated to $B_1'$ and $B_2'$ 
so that $\E[\beta_1 \mathbf{1}_{B_1'} + \beta_2 \mathbf{1}_{B_2'}] = \beta_1 \mathbf{1}_{B_1} + \beta_2 \mathbf{1}_{B_2}$, 
which is a key property to show the validity of the algorithm. 


The most time consuming part in \texttt{MergeBases} is to find a pair of elements $u$ and $v$ 
satisfying the above conditions. 
% $u \in B_1 \setminus B_2$
% and $v \in B_2 \setminus B_1$ such that $B_1 + v - u \in \I$ and $B_2 + u - v \in \I$. 
By the strong basis exchange property of matroids, 
we can find such a pair of elements using $O(r)$ independence oracle queries in the following way: 
fix an element $u\in B_1 \setminus B_2$ arbitrarily and 
check the conditions for each element $v \in B_2 \setminus B_1$ one by one. 
Since we update the bases $|B_1 \setminus B_2| = O(r)$ times, 
\texttt{MergeBases} requires $O(r^2)$ independence oracle queries in total.
Hence, \texttt{SwapRound} requires $O(r^2 t)$ independence oracle queries. 

It is not clear whether we can develop an algorithm that finds such a pair of elements $u$ and $v$ using $o(r)$ independence oracle queries.
Therefore, their implementation of \texttt{SwapRound} is now stuck at $\Omega(r^2 t)$ independence oracle queries.
%Therefore, their implementation of \texttt{MergeBases} is now stuck at $\Omega(r^2)$ independence oracle queries.


%Our goal in this section is to present the merge bases algorithm that uses $o(r)$ independence oracle queries in a single execution.


% {\bf TODO: We want to describe the desired property of the output.}

% {\bf TODO: Describe a key to show such a property.}


%%{\bf TODO: Should we merge Algo 2 and 3?}


% see Algorithms~\ref{alg:mergebases}~\ref{alg:update_via_strong_basis_exchange}

% the procedure \texttt{MergeBases} (Algorithm \ref{alg:mergebases})




% The implementation given by Chekuri et al. uses $O(r^2 t)$ independence oracle queries, where $r$ is the rank of the matroid $\M$ and $t$ is the number of bases in the representation of $x$.
% In their algorithm, we apply the procedure \texttt{MergeBases} (Algorithm \ref{alg:mergebases}) $t - 1$ times.


% Given two bases $B_1$ and $B_2$, the procedure \texttt{MergeBases} creates a new base $C_2$ from the elements in $B_1 \cup B_2$.

% In their implementation of the merge bases algorithm, 
% we are given an element $v \in B_1 \setminus B_2$ and need to find an element $u \in B_2 \setminus B_1$ such that $B_1 + v - u \in \I$ and $B_2 + u - v \in \I$.
% We check all elements in $B_2 \setminus B_1$ to find such element, which uses $O(r)$ independece oracle queries.
% It is not clear whether we can develop an algorithm that finds a suitable element using $o(r)$ independence oracle queries.
% Then, their implementation of the merge bases algorithm are now stuck at $\Omega(r)$ independence oracle queries.
% Then 

% Our goal in this section is to present the merge bases algorithm that uses $o(r)$ independence oracle queries in a single execution.

% \begin{theorem} \label{thm:fast_swap_rounding}
% There is a randomized algorithm that takes as input a fractional solution $x$ represented as a covex combination of $t$ bases and rounds it to an integral solution $S$ such that $\E[f(S)] \geq F(x)$.
% This algorithm uses $O(r^{3/2}t \log^2(r t))$ independence oracle queries with high probability, where $r$ is the rank of $\M$.
% \end{theorem}

% \begin{corollary} \label{cor:fast_swap_rounding}
% There is a randomized algorithm that takes as input a fractional solution $x$ represented as a covex combination of $t$ bases and rounds it to an integral solution $S$ such that $\E[f(S)] \geq (1 - \epsilon) F(x)$.
% This algorithm uses $\displaystyle O\left(r^{3/2}t \log^2\left(\frac{rt}{\epsilon}\right)\right)$ independence oracle queries.
% \end{corollary}

% \begin{proof}[Proof of Corollary \ref{cor:fast_swap_rounding}]
% \end{proof}

\begin{algorithm} %[H]
    $C_1 \gets B_1$ \\
    $\gamma_1 \gets \beta_1$ \\
    \For{$i = 1$ \textup{to} $t - 1$} {
        $C_{i + 1} \gets \text{\texttt{MergeBases}}(\gamma_i, C_i, \beta_{i + 1}, B_{i + 1})$ \\
        $\gamma_{i + 1} \gets \gamma_i + \beta_{i + 1}$ \\
    }
    \Return $C_t$
    \caption{\texttt{SwapRound}$(x = \sum_{i = 1}^{t} \beta_i \mathbf{1}_{B_i})$}\label{alg:swapround}
\end{algorithm}

\begin{algorithm} %[H]
    \While {$B_1 \neq B_2$} {
        Pick arbitrary $u \in B_1 \setminus B_2$ \\
        Find $v \in B_2 \setminus B_1$ such that $B_1 + v - u \in \I$ and $B_2 + u - v \in \I$ \label{line:mergebases_1} \\
        % Flip a coin with \texttt{Heads} probability $\displaystyle \frac{\beta_1}{\beta_1 + \beta_2}$ \\
        % \If{coin flipped \textup{\texttt{Heads}}} {
        %     $B_2 \gets B_2 + u - v$
        % } \Else {
        %     $B_1 \gets B_1 + v - u$
        % }
        \texttt{UpdateViaStrongBasisExchange}$(\beta_1, B_1, \beta_2, B_2, v, u)$ \\
    } 
    \Return $B_1$
    \caption{\texttt{MergeBases}$(\beta_1, B_1, \beta_2, B_2)$}\label{alg:mergebases}
\end{algorithm}

\begin{algorithm} %[H]
    \KwIn{$\beta_1, \beta_2 \in \mathbb{R}_{+}$, two bases $B_1, B_2$, and elements $v \in B_2 \setminus B_1$ and $u \in B_1 \setminus B_2$  such that $B_1 + v - u \in \I$ and $B_2 + u - v \in \I$}
    Flip a coin with \texttt{Heads} probability $\displaystyle \frac{\beta_2}{\beta_1 + \beta_2}$ \\
    \If{coin flipped \textup{\texttt{Heads}}} {
        $B_1 \gets B_1 + v - u$
    } \Else {
        $B_2 \gets B_2 + u - v$
    }
    \caption{\texttt{UpdateViaStrongBasisExchange}$(\beta_1, B_1, \beta_2, B_2, v, u)$}\label{alg:update_via_strong_basis_exchange}
\end{algorithm}
